Optimal Planning for Timed Partial Order Specifications

This paper addresses the challenge of planning a sequence of tasks to be performed by multiple robots while minimizing the overall completion time subject to timing and precedence constraints. Our approach uses the Timed Partial Orders (TPO) model to specify these constraints. We translate this problem into a Traveling Salesman Problem (TSP) variant with timing and precedent constraints, and we solve it as a Mixed Integer Linear Programming (MILP) problem. Our contributions include a general planning framework for TPO specifications, a MILP formulation accommodating time windows and precedent constraints, its extension to multi-robot scenarios, and a method to quantify plan robustness. We demonstrate our framework on several case studies, including an aircraft turnaround task involving three Jackal robots, highlighting the approach's potential applicability to important real-world problems. Our benchmark results show that our MILP method outperforms state-of-the-art open-source TSP solvers OR-Tools.

==> reviews.tex <==
%auto-ignore
\section{Important Reviews}
\subsection{Reviewer 1}

\begin{itemize}
    \item No guide on how to avoid collisions.
    \item What if any delay or failure occurred.
    \item Figure 5 is hard to follow.
    \item Figure 6 is too small
\end{itemize}


\subsection{Reviewer 2}

\begin{itemize}
    \item computational efficiency gains compared to what?
    \item The strength of your formulation as opposed to STL is not emphasized enough.
    \item As for the related work on task allocation, it is worded strange because afterwards I'm still not sure whether tasks are assigned to robots or they are not
    \item in the footnote 1, what is $\sigma$? shouldn't it be $L(s,\gamma_k)$?
    \item Def 3. and/or 4. would become stronger with a (running) example. (Maybe for the thesis!!!)

    \item Mention Time-robust STL motion planning in the related work section.
    \item (Video) Conclusion is too short. Perhaps you could also include some of the drawbacks that you think of addressing in future work.
\end{itemize}


\subsection{Reviewer 3}

\begin{itemize}
    \item The authors should compare it to more advanced baselines such as local search, Multiple vehicle rouging problem with time windows, or even greedy planners.
    \item The translation of such a constrained optimization problem into integer optimization is a standard approach and would be the first thing to try. 
    \item Clearly state the novelty and contributions w.r.t. the current state of the art
    \item taking into account more recent baselines such as MVRPTW and Local search solvers for large-scale systems and different numbers of tasks.
\end{itemize}


\section{Conclusion}
\begin{itemize}
    \item Explain how collisions can be avoided
    \item What's new about this paper? -> local and global timing constraints make the problem difficult. Show experiments against ORTools.
    \item 
\end{itemize}


==> sections/06_Experiments/tpo2.tex <==
\begin{tikzpicture}
\matrix[every node/.style={draw=black, rectangle, rounded corners, font=\small}, row sep=6pt, column sep=8pt]{
                        & \node(n4){$e_{green}$}; & \node(n5){$e_{yellow}$}; & \node(n6){$e_{blue}$}; \\
 \node(n1){$e_{init}$}; & \node(n2){$e_{grey}$}; & \node(n3){$e_{red}$}; &\\
                        & & \node(n7){$e_{purple}$}; && \\
};
\path[->, line width=1pt] (n1) edge (n2)
                          (n2) edge (n3)
                          (n3) edge (n6)
                          (n1) edge (n4)
                          (n4) edge (n5)
                          (n5) edge (n6)
                          (n2) edge (n7);
                          
\draw (n1.north)++(0,0.3) node {$c_1:=0$};
\draw (n2.south)++(-0.2,-0.2) node {$20 \leq c_1 \leq 30$};
\draw (n3.east)++(0.2,-0.2) node {$c_4:=0$};
\draw (n4.north)++(-0.3,0.3) node {$c_1 \leq 20$, $c_2:=0$};
\draw (n5.north)++(0,0.3) node {$5\leq c_2\leq30, c_3:=0$};
\draw (n6.south)++(0,-0.3) node {$0 \leq c_3 \leq 40 \land 0 \leq c_4 \leq 10$};
\draw (n7.south)++(0,-0.3) node {$c_3\leq40 \land c_4\leq10$};

\end{tikzpicture}


==> sections/06_Experiments/tpo_minigrid_.tex <==
\begin{tikzpicture}
\matrix[every node/.style={draw=black, rectangle, rounded corners, font=\small}, row sep=5pt, column sep=7pt]{
                        & \node(n4){$e_{yellow}$}; & \node(n5){$e_{blue}$}; & \node(n6){$e_{red}$}; \\
 \node(n1){$e_{init}$}; & \node(n2){$e_{grey}$}; & \node(n3){$e_{purple}$}; &&\\
};
\path[->, line width=1pt] (n1) edge (n2)
(n2) edge (n3)
(n2) edge (n4)
(n4) edge (n5)
(n5) edge (n6);
\draw (n1.north)++(0,0.3) node {$c_1 := 0$};
\draw (n2.south)++(0,-0.3) node {$20 \leq c_1 \leq 30$};
\draw (n4.north)++(0,0.3) node {$c_2 := 0$};
\draw (n5.north)++(0,0.3) node {$c_2 \leq 10$};
\draw (n6.east)++(0.8,-0.3) node {$50 \leq c_1 \leq 60$};
\end{tikzpicture}

